VerifiedLab: Harnessing Knowns for Unknowns

Across human history, knowledge has undergone several transitions, from orality to writing and then to digital archives. At each transition, humans established new conventions to preserve knowledge for the new era. Nowadays, as research agents are increasingly deployed for laboratory experiments, knowledge is crossing another boundary: from records written for humans to those for machines. In this work, we introduce VerifiedLab, a multi-agent harness framework for this human-to-machine transition of knowledge. VerifiedLab transforms research output from passive artifacts into active systems that accelerate downstream use, adoption and prediction of future trends. In VerifiedLab, a team of AI scientists with distinct roles reasons over records verified field by field: a principal investigator plans, a librarian computes the evidence directly from the records, specialists draft, and a gate and a critic check each claim against the measured reliability of its data before the harness decides whether to release or withhold it. We demonstrate the efficacy of VerifiedLab through extensive experiments on perovskite solar cells: VerifiedLab recovers known physical trends, anticipates devices reported a year later, and lets AI scientists inherit the literature together with a measure of how far it can be trusted. By scaling the inference-time verification compute, VerifiedLab introduces a new pathway for knowledge dissemination and machine harness for AI co-scientists.

==> supp_labels.tex <==
\makeatletter
% Generated by scripts/sync_xrefs.py from supplementary.aux; do not edit.
\xr@def{S}{fig:database}{4}
\xr@def{S}{fig:ed-generators}{1}
\xr@def{S}{fig:ed-subfields}{2}
\xr@def{S}{fig:ed-verifiers}{3}
\xr@def{S}{fig:pred-tabular}{5}
\xr@def{S}{fig:pred-text}{6}
\xr@def{S}{fig:ws-claims}{13}
\xr@def{S}{fig:ws-data}{11}
\xr@def{S}{fig:ws-literature}{8}
\xr@def{S}{fig:ws-overview}{7}
\xr@def{S}{fig:ws-reliability}{10}
\xr@def{S}{fig:ws-session}{12}
\xr@def{S}{fig:ws-skills}{15}
\xr@def{S}{fig:ws-studio}{9}
\xr@def{S}{fig:ws-trace}{14}
\xr@def{S}{tab:scale-vs-skill}{2}
\xr@def{S}{tab:verifier-acceptance}{1}
\makeatother

